Reliable Tests of Faint-end UV Luminosity Functions in Strong Lensing Fields

Dark matter comprises ~85% of the entire mass of the Universe, but the fundamental nature of its constituent particles remains elusive. In this thesis, I test for two competitive dark matter models: the conventional heavy particle paradigm, and dark matter being ultralight bosons of mass $\sim 10^{-22}$eV ($\psi$DM). More specifically, I test for the faint-end turnover induced by $\psi$DM models, exploiting the strong lensing power by massive galaxy clusters to probe intrinsically fainter magnitudes. A key challenge for such an analysis would be contamination by low-z galaxies sharing similar observed SEDs as high-z galaxies. As I will demonstrate, such a contamination issue is generally severe and may wash out the faint-end turnover signatures. I also show that $\sim 50\%$ of the purported $3.5\leq z\leq 5.5$ galaxies within existing photometric redshift catalogs constructed for Hubble Frontier Fields (HFF) are in fact low-z interlopers. Luckily, individual mitigation of interlopers can be achieved with the combination of deep HST and JWST observations. For fields without supplementary data, machine learning methods will be shown useful in preserving the mitigating power. Cleaner $3.5\leq z\leq 5.5$ and $6\leq z\leq 10$ samples are derived for a more reliable test in strong lensing field of MACS J0416, with which I found no evidence for faint-end turnovers, leading to a constraint on the $\psi$DM mass of $>2.97\times10^{-22}$eV at 95\% confidence. This constraint will also be interpreted in an scheme where dark matter is composed of multiple particle copies, where I argue the derived mass bound is likely on an effective de Broglie scale governing the collective behavior of the entire $\psi$DM budget under gravitational equilibrium established.

==> Chapters/Chapter1.tex <==
% Chapter 1

\chapter{Introduction} % Main chapter title

\label{Chapter1} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
% \newcommand{\keyword}[1]{\textbf{#1}}
% \newcommand{\tabhead}[1]{\textbf{#1}}
% \newcommand{\code}[1]{\texttt{#1}}
% \newcommand{\file}[1]{\texttt{\bfseries#1}}
% \newcommand{\option}[1]{\texttt{\itshape#1}}

%----------------------------------------------------------------------------------------

% =========================================================== %
%                 Section: General Information                %
% =========================================================== %
\section{General Information}
\label{chap1:sec1:general_information}
This template is for MPhill/Doctor students of University of Hong Kong to prepare their theses. The entire project strictly follows the requirements of \uline{booklet provided by Graduate School of the University of Hong Kong}. The current version of this template is prepared according to the $\boldsymbol{13^\mathrm{th}}$ edition of the booklet entitled ``\href{https://intraweb.hku.hk/reserved_1/gradsch/PreparingandSubmittingYourThesis.pdf}{Preparing and Submitting Your Thesis --- A Guide for MPhil and PhD Students.}'' This edition is updated in \textbf{July 2019}. Considering the university may change the stipulations over time, this template also provides the guidelines to adjust the typeset. The current version of the template has been tested by the author(s) and has been successfully accepted by the Engineering Faculty.
However, \uline{users should also notice that this is not an official template, and we are not responsible for any problems of your thesis preparation and submission caused by using this template.} For anyone who would like to use this template, you have to be responsible for your thesis and your are supposed to carefully read and follow the rules in the latest edition of the university booklet to prepare your thesis. In the rest of the template, we will demonstrate how to use, change, or adjust this template.


% =========================================================== %
%      Section: General Requirements of Graduate School       %
% =========================================================== %
\section{General Requirements of Graduate School}
\label{chap1:sec2:general_requirements_of_graduate_school}
According to the \href{https://intraweb.hku.hk/reserved_1/gradsch/PreparingandSubmittingYourThesis.pdf}{$13^\mathrm{th}$ edition booklet}, ``The Thesis Format'' section, the thesis submitted for examination shall be typewritten or printed on one side or both sides of International size A4 paper, with a margin of not less than 35mm on both right and left-hand edges of each page (as shown in \figref{fig:chap1:thesis_requirements}).
\begin{figure}[!h]
    \centering
    \includegraphics[width=.96\textwidth]{Figures/Chapter1/thesis_requirement.PNG}
    \caption{Requirements of the thesis format in the Graduate School $13^\mathrm{th}$ edition booklet at Page 9.}
    \label{fig:chap1:thesis_requirements}
\end{figure}


% =========================================================== %
%                    Subsection: Page Margin                  %
% =========================================================== %
\subsection{Page Margin}
\label{chap1:sec:2:subsec1:page_margin}
The format of page size and margin is defined in ``main.tex'' file \textbf{Line 63-71}. The page margin of the current version template is \uline{Left: 35mm, Right: 36mm (a4paper).} Users can change the page margin by adjusting the corresponding settings. There is no stipulation for the top and bottom margins, but the booklet recommend that both of them should be 25mm, which is adopted in this template. 


% =========================================================== %
%          Subsection: Font, Alignment, Line Spacing          %
% =========================================================== %
\subsection{Font, Alignment, Line Spacing}
Ordinarily, there is no restrict stipulation for the font family, font size, alignment, and line spacing. All of these are a matter of personal preference. This template uses \textit{10pt} font size, \textit{Fully Justified} alignment style and \textit{One and A Half} line spacing. Users can adjust the settings in \textbf{Line 19-33} of the ``main.tex'' file to change the typeset.


% =========================================================== %
%                      Subsection: Contents                   %
% =========================================================== %
\subsection{Contents}
The contents of this template can be subdivided into three parts --- the front matter, the text and the back matter, which strictly follows the stipulations of the official booklet (Page 17). \tabref{chap1:longtable:checking_list} indicates the what contents are required in the submitted thesis and what contents are optional. The column ``Required'' denotes that 
\begin{center}
\begin{longtable}{|l|c|c|}
\caption{Checking list indicating the contents should be included in the thesis.}\label{chap1:longtable:checking_list}\\
\hline
\textbf{The Front Matter} & Required     &  Include $\checkmark$ \\ \hline \hline
Abstract                  & Yes          & $\checkmark$         \\
Title Page                & Yes          & $\checkmark$         \\
Frontispiece              &              &                      \\
Dedication                &              & $\checkmark$         \\
Epigraph                  &              &                      \\
Declarations              & Yes          & $\checkmark$         \\
Acknowledgements          &              & $\checkmark$         \\
Table of Contents         & Yes          & $\checkmark$         \\
List of Illustrations     &              &                      \\
List of Figures           &              & $\checkmark$         \\
List of Tables            &              & $\checkmark$         \\
List of Algorithm         &              & $\checkmark$         \\
List of Abbreviations     &              & $\checkmark$         \\
List of Symbols           &              & $\checkmark$         \\
Others                    &              &                      \\ \hline \hline
\textbf{The Text}         & Yes          & $\checkmark$         \\ \hline \hline
\textbf{The Reference or Back Matter} &    ---    &   ---       \\ \hline \hline
Glossary                  &              &                      \\
Appendices                &              &                      \\
Notes                     &              &                      \\
Bibliography or Reference List & Yes          &  $\checkmark$   \\
Index                     &              &                      \\
\hline
\end{longtable}
\end{center}
This template support most of the contents listed in the figure, including the ``Abstract'', ``Title Page'', ``Declarations'', ``Acknowledgements'', ``List of Publications'', ``Contents'', ``List of Figures'', ``List of Tables'', ``List of Algorithms'', ``List of Abbreviations'', ``List of Symbols'', ``Main Text'', ``Appendices'', and ``Bibliography''. Each part is defined in an independent tex file and the ``main.tex'' file combines all the different parts to form the entire thesis. Therefore, users can easily make the changes by adjusting the corresponding document files.

In addition to the stipulations of the booklet, this template also provides a beautiful \textbf{cover page}, which is the first two pages of this project. \uline{The cover page is \textbf{not required} by the Graduate School and you'd better remove the cover page when bounding your thesis for submission.}










==> Chapters/Chapter2.tex <==
% Chapter 2

\chapter{Guidelines on Adjustments} % Main chapter title

\label{Chapter2} % For referencing the chapter elsewhere, use \ref{Chapter2} 

%----------------------------------------------------------------------------------------

% Define some commands to keep the formatting separated from the content 
% \newcommand{\keyword}[1]{\textbf{#1}}

%----------------------------------------------------------------------------------------
This chapter demonstrates how to make changes and DIY the thesis style when using this template. For each component of the thesis, we provide both 

\section{Title Page}
\textbf{Title Page} is designed to obviously bear the title of the thesis and the author's name. Users can add any degrees or professional qualifications that he/she holds as well as the author's name in the national script. Both the title and the author's name are highlighted in blod style. Given that there may also be an oral and/or written examination, and thus this template uses the following form of words:

\begin{quote}
A thesis submitted in partial fulfilment of the requirements for the degree of Doctor (or Master) of Philosophy at The University of Hong Kong.
\end{quote}

\noindent The title page is not numbered, or counted in the pagination of the front mater, or listed in the table of contents. The document for title page is quite simple, which can be found in the path \colorbox{gray!20}{Titlepage/titlepage.tex}.


\section{Dedication}
\label{chap2:sec2:dedication}
\textbf{Dedication} is a place to show your wish to dedicate the thesis to friends, family or loved ones. This template uses a single page example for dedication, as shown in \figref{fig:chap2:dedication_sample}. This page is not numbered, or counted in the pagination of the front matter, or listed in the table of contents.
\begin{figure}
    \centering
    \includegraphics[width=.6\textwidth]{Dedication/dedication.pdf}
    \caption{An example dedication page.}
    \label{fig:chap2:dedication_sample}
\end{figure}


\section{Epigraph}
\label{chap2:sec3:epigraph}
\textbf{Epigraph} is a relevant quotation on the subject of the thesis, or some general guidelines or philosophical principles. Ordinarily, the author and source of the quotation should also be given. This page is not included in the template and users can add the epigraph page according to their willingness.


\section{Declarations}
\label{chap2:sec4:declarations}
\textbf{Declarations} page is a required item according to the official booklet. The contents of declaration are in terms of the official sample (\textit{Sample Page 6} on page 41 of the booklet) with some minor changes to specify the author's name and thesis title.


\section{Acknowledgements}
\label{chap2:sec5:acknowledgements}
\textbf{Acknowledgements} is the place where the author thanks mentors, labmates, colleagues, friends, family members and also the financial support from scholarships and research grants. Each page of the acknowledgements is numbered in lower case Roman numerals


\section{Table of Contents}
\label{chap2:sec6:table_of_contents}
\textbf{Table of Contents} in this template is simply headed ``Contents'' which lists all the parts of the thesis and the page on which they commence. Each of the chapters, sections and subsections are included in the list. The capitalization and wording of the titles listed in the table exactly agree with the corresponding ones appear in the body text. If users would like to include some optional pages in the Table of Contents, such as the Frontispiece page or Epigraph page, they can simply add a command \verb|\addchaptertocentry{\pagename}| at the corresponding page. For example, your can add the \textit{Abstract} item to the Table of Contents, by adding the command to the file \codestyle{Abstract/abstract.tex}, as shown in \figref{fig:chap2:example_add_command}.
\begin{figure}[!h]
    \centering
    \includegraphics[width=.8\textwidth]{Figures/Chapter2/add_command_example.png}
    \caption{An example of how to add chapter to the Table of Contents.}\label{fig:chap2:example_add_command}
\end{figure}


\section{List of Tables, Figures and Algorithms, etc}
\label{chap2:sec7:list_of_tables_figures_and_algorithms_etc}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/Chapter2/photo_consistency.pdf}
    \caption{Light transformation model in a plenoptic camera. Within a plenoptic camera, a micro-lens array has been placed at the image plane, which further splits the incoming light rays from different directions and records them separately. Therefore, the multi-view information can be extracted from each light field image captured by a single shot.}
    \label{fig:photo_consistency}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/Chapter2/photo_consistency.pdf}
    \caption[Light transformation model (focused on the plane).]{Light transformation model in a plenoptic camera. Within a plenoptic camera, a micro-lens array has been placed at the image plane, which further splits the incoming light rays from different directions and records them separately. Therefore, the multi-view information can be extracted from each light field image captured by a single shot.}
    \label{fig:photo_consistency_with_nickname}
\end{figure}
Following the Table of Contents, the template includes the lists of tables, figures and algorithms, abbreviations and symbols. The numbering, capitalisation and wording of the titles of every items listed agree exactly with the manner in which they appear in the body text. For the illustration with a long title, users can also provide a ``nickname'' of the illustration by enclosing the it in the square brackets. For example, \figref{fig:photo_consistency} and \figref{fig:photo_consistency_with_nickname} have the same image captions in the body text, but the wordings appear in the Table of Contents are different. \figref{fig:photo_consistency_with_nickname} uses the wordings in the square brackets as its caption, as shown at page \darkred{vii}.

